One-loop contributions to decays $e_b\to e_a \gamma$ and $(g-2)_{e_a}$ anomalies, and Ward identity

In this paper, we will present analytic formulas to express one-loop contributions to lepton flavor violating decays $e_b\to e_a \gamma$, which are also relevant to the anomalous dipole magnetic moments of charged leptons $e_a$. These formulas were computed in the unitary gauge, using the well-known Passarino-Veltman notations. We also show that our results are consistent with those calculated previously in the 't Hooft-Veltman gauge, or in the limit of zero lepton masses. At the one-loop level, we show that the appearance of fermion-scalar-vector type diagrams in the unitary gauge will violate the Ward Identity relating to an external photon. As a result, the validation of the Ward Identity guarantees that the photon always couples with two identical particles in an arbitrary triple coupling vertex containing a photon.

==> bibilio.tex <==
\bibitem{Muong-2:2021ojo}
B.~Abi \textit{et al.} [Muon g-2],
%``Measurement of the Positive Muon Anomalous Magnetic Moment to 0.46 ppm,''
Phys. Rev. Lett. \textbf{126}, no.14, 141801 (2021)
%doi:10.1103/PhysRevLett.126.141801
%[arXiv:2104.03281 [hep-ex]].

\bibitem{Aoyama:2020ynm}
T.~Aoyama, N.~Asmussen, M.~Benayoun, J.~Bijnens, T.~Blum, M.~Bruno, I.~Caprini, C.~M.~Carloni Calame, M.~C\`e and G.~Colangelo, \textit{et al.}
%``The anomalous magnetic moment of the muon in the Standard Model,''
Phys. Rept. \textbf{887}, 1 (2020)
%doi:10.1016/j.physrep.2020.07.006
%[arXiv:2006.04822 [hep-ph]].
%

\bibitem{Keshavarzi:2018mgv}
A.~Keshavarzi, D.~Nomura and T.~Teubner,
%``Muon $g-2$ and $\alpha(M_Z^2)$: a new data-based analysis,''
Phys. Rev. D \textbf{97}, no.11, 114025 (2018)
%doi:10.1103/PhysRevD.97.114025
[arXiv:1802.02995 [hep-ph]].

\bibitem{Colangelo:2018mtw}
G.~Colangelo, M.~Hoferichter and P.~Stoffer,
%``Two-pion contribution to hadronic vacuum polarization,''
JHEP \textbf{02}, 006 (2019)
%doi:10.1007/JHEP02(2019)006
[arXiv:1810.00007 [hep-ph]].

\bibitem{Hoferichter:2019mqg}
M.~Hoferichter, B.~L.~Hoid and B.~Kubis,
%``Three-pion contribution to hadronic vacuum polarization,''
JHEP \textbf{08}, 137 (2019)
%doi:10.1007/JHEP08(2019)137
[arXiv:1907.01556 [hep-ph]].

\bibitem{Davier:2019can}
M.~Davier, A.~Hoecker, B.~Malaescu and Z.~Zhang,
%``A new evaluation of the hadronic vacuum polarisation contributions to the muon anomalous magnetic moment and to $\mathbf{\boldsymbol\alpha(m_Z^2)}$,''
Eur. Phys. J. C \textbf{80}, no.3, 241 (2020)
[erratum: Eur. Phys. J. C \textbf{80}, no.5, 410 (2020)]
%doi:10.1140/epjc/s10052-020-7792-2
[arXiv:1908.00921 [hep-ph]].
%
\bibitem{Keshavarzi:2019abf}
A.~Keshavarzi, D.~Nomura and T.~Teubner,
%``$g-2$ of charged leptons, $\alpha (M^2_Z)$ , and the hyperfine splitting of muonium,''
Phys. Rev. D \textbf{101}, no.1, 014029 (2020)
%doi:10.1103/PhysRevD.101.014029
[arXiv:1911.00367 [hep-ph]].

\bibitem{Kurz:2014wya}
A.~Kurz, T.~Liu, P.~Marquard and M.~Steinhauser,
%``Hadronic contribution to the muon anomalous magnetic moment to next-to-next-to-leading order,''
Phys. Lett. B \textbf{734}, 144-147 (2014)
%doi:10.1016/j.physletb.2014.05.043
[arXiv:1403.6400 [hep-ph]].


\bibitem{Melnikov:2003xd}
K.~Melnikov and A.~Vainshtein,
%``Hadronic light-by-light scattering contribution to the muon anomalous magnetic moment revisited,''
Phys. Rev. D \textbf{70}, 113006 (2004)
%doi:10.1103/PhysRevD.70.113006
[arXiv:hep-ph/0312226 [hep-ph]].

%[19] P. Masjuan and P. Sanchez-Puertas, ´ Phys. Rev. D95, 054026 (2017), arXiv:1701.05829 [hep-ph].
\bibitem{Masjuan:2017tvw}
P.~Masjuan and P.~Sanchez-Puertas,
%``Pseudoscalar-pole contribution to the $(g_{\mu}-2)$: a rational approach,''
Phys. Rev. D \textbf{95}, no.5, 054026 (2017)
%doi:10.1103/PhysRevD.95.054026
[arXiv:1701.05829 [hep-ph]].

%[20] G. Colangelo, M. Hoferichter, M. Procura, and P. Stoffer, JHEP 04, 161 (2017), arXiv:1702.07347 [hep-ph]
\bibitem{Colangelo:2017fiz}
G.~Colangelo, M.~Hoferichter, M.~Procura and P.~Stoffer,
%``Dispersion relation for hadronic light-by-light scattering: two-pion contributions,''
JHEP \textbf{04}, 161 (2017)
%doi:10.1007/JHEP04(2017)161
[arXiv:1702.07347 [hep-ph]].

%[21] M. Hoferichter, B.-L. Hoid, B. Kubis, S. Leupold, and S. P. Schneider, JHEP 10, 141 (2018), arXiv:1808.04823 [hep-ph].

\bibitem{Hoferichter:2018kwz}
M.~Hoferichter, B.~L.~Hoid, B.~Kubis, S.~Leupold and S.~P.~Schneider,
%``Dispersion relation for hadronic light-by-light scattering: pion pole,''
JHEP \textbf{10}, 141 (2018)
%doi:10.1007/JHEP10(2018)141
[arXiv:1808.04823 [hep-ph]].

%[22] A. Gerardin, H. B. Meyer, and A. Ny ´ ffeler, Phys. Rev. D100, 034520 (2019), arXiv:1903.09471 [hep-lat].  
\bibitem{Gerardin:2019vio}
A.~G\'erardin, H.~B.~Meyer and A.~Nyffeler,
%``Lattice calculation of the pion transition form factor with $N_f=2+1$ Wilson quarks,''
Phys. Rev. D \textbf{100}, no.3, 034520 (2019)
%doi:10.1103/PhysRevD.100.034520
[arXiv:1903.09471 [hep-lat]].

%[23] J. Bijnens, N. Hermansson-Truedsson, and A. Rodr´ıguez-Sanchez, ´ Phys. Lett. B798, 134994 (2019), arXiv:1908.03331 [hep-ph].

\bibitem{Bijnens:2019ghy}
J.~Bijnens, N.~Hermansson-Truedsson and A.~Rodr\'\i{}guez-S\'anchez,
%``Short-distance constraints for the HLbL contribution to the muon anomalous magnetic moment,''
Phys. Lett. B \textbf{798}, 134994 (2019)
%doi:10.1016/j.physletb.2019.134994
[arXiv:1908.03331 [hep-ph]].

%[24] G. Colangelo, F. Hagelstein, M. Hoferichter, L. Laub, and P. Stoffer, JHEP 03, 101 (2020), arXiv:1910.13432 [hep-ph].
\bibitem{Colangelo:2019uex}
G.~Colangelo, F.~Hagelstein, M.~Hoferichter, L.~Laub and P.~Stoffer,
%``Longitudinal short-distance constraints for the hadronic light-by-light contribution to $(g-2)_\mu$ with large-$N_c$ Regge models,''
JHEP \textbf{03}, 101 (2020)
%doi:10.1007/JHEP03(2020)101
[arXiv:1910.13432 [hep-ph]].

%[31] G. Colangelo, M. Hoferichter, A. Nyffeler, M. Passera, and P. Stoffer, Phys. Lett. B735, 90 (2014), arXiv:1403.7512 [hep-ph]
\bibitem{Colangelo:2014qya}
G.~Colangelo, M.~Hoferichter, A.~Nyffeler, M.~Passera and P.~Stoffer,
%``Remarks on higher-order hadronic corrections to the muon g\ensuremath{-}2,''
Phys. Lett. B \textbf{735}, 90-91 (2014)
%doi:10.1016/j.physletb.2014.06.012
[arXiv:1403.7512 [hep-ph]].

%[32] T. Blum, N. Christ, M. Hayakawa, T. Izubuchi, L. Jin, C. Jung, and C. Lehner, Phys. Rev. Lett. 124, 132002 (2020), arXiv:1911.08123
\bibitem{Blum:2019ugy}
T.~Blum, N.~Christ, M.~Hayakawa, T.~Izubuchi, L.~Jin, C.~Jung and C.~Lehner,
%``Hadronic Light-by-Light Scattering Contribution to the Muon Anomalous Magnetic Moment from Lattice QCD,''
Phys. Rev. Lett. \textbf{124}, no.13, 132002 (2020)
%doi:10.1103/PhysRevLett.124.132002
[arXiv:1911.08123 [hep-lat]].

%[33] T. Aoyama, M. Hayakawa, T. Kinoshita, and M. Nio, Phys. Rev. Lett. 109, 111808 (2012), arXiv:1205.5370 [hep-ph].
\bibitem{Aoyama:2012wk}
T.~Aoyama, M.~Hayakawa, T.~Kinoshita and M.~Nio,
%``Complete Tenth-Order QED Contribution to the Muon g-2,''
Phys. Rev. Lett. \textbf{109}, 111808 (2012)
%doi:10.1103/PhysRevLett.109.111808
[arXiv:1205.5370 [hep-ph]].

%[34] T. Aoyama, T. Kinoshita, and M. Nio, Atoms 7, 28 (2019).
\bibitem{Aoyama:2019ryr}
T.~Aoyama, T.~Kinoshita and M.~Nio,
%``Theory of the Anomalous Magnetic Moment of the Electron,''
Atoms \textbf{7}, no.1, 28 (2019)
%doi:10.3390/atoms7010028

%[35] A. Czarnecki, W. J. Marciano, and A. Vainshtein, Phys. Rev. D67, 073006 (2003), [Erratum: Phys. Rev. D73, 119901 (2006)], arXiv:hepph/0212229 [hep-ph].
\bibitem{Czarnecki:2002nt}
A.~Czarnecki, W.~J.~Marciano and A.~Vainshtein,
%``Refinements in electroweak contributions to the muon anomalous magnetic moment,''
Phys. Rev. D \textbf{67}, 073006 (2003)
[erratum: Phys. Rev. D \textbf{73}, 119901 (2006)]
%doi:10.1103/PhysRevD.67.073006
[arXiv:hep-ph/0212229 [hep-ph]].

%[36] C. Gnendiger, D. Stockinger, and H. St ¨ ockinger-Kim, ¨ Phys. Rev. D88, 053005 (2013), arXiv:1306.5546 [hep-ph]
\bibitem{Gnendiger:2013pva}
C.~Gnendiger, D.~St\"ockinger and H.~St\"ockinger-Kim,
%``The electroweak contributions to $(g-2)_\mu$ after the Higgs boson mass measurement,''
Phys. Rev. D \textbf{88}, 053005 (2013)
%doi:10.1103/PhysRevD.88.053005
[arXiv:1306.5546 [hep-ph]].

%%%new references from communications, updated 19, Sep, 2021
%------Bogdan Malaescu,

%\bibitem{Davier:2019can}

\bibitem{Davier:2017zfy}
M.~Davier, A.~Hoecker, B.~Malaescu and Z.~Zhang,
%``Reevaluation of the hadronic vacuum polarisation contributions to the Standard Model predictions of the muon $g-2$ and ${\alpha (m_Z^2)}$ using newest hadronic cross-section data,''
Eur. Phys. J. C \textbf{77}, no.12, 827 (2017)
%doi:10.1140/epjc/s10052-017-5161-6
[arXiv:1706.09436 [hep-ph]].



\bibitem{Davier:2010nc}
M.~Davier, A.~Hoecker, B.~Malaescu and Z.~Zhang,
%``Reevaluation of the Hadronic Contributions to the Muon g-2 and to alpha(MZ),''
Eur. Phys. J. C \textbf{71}, 1515 (2011)
[erratum: Eur. Phys. J. C \textbf{72}, 1874 (2012)]
%doi:10.1140/epjc/s10052-012-1874-8
[arXiv:1010.4180 [hep-ph]].
%--------------end 19 Sep 2021


\bibitem{Morel:2020dww}
L.~Morel, Z.~Yao, P.~Clad\'e and S.~Guellati-Kh\'elifa,
%``Determination of the fine-structure constant with an accuracy of 81 parts per trillion,''
Nature \textbf{588}, no.7836, 61-65 (2020)
%doi:10.1038/s41586-020-2964-7


\bibitem{MEG:2016leq}
A.~M.~Baldini \textit{et al.} [MEG],
%``Search for the lepton flavour violating decay $\mu ^+ \rightarrow \mathrm {e}^+ \gamma $ with the full dataset of the MEG experiment,''
Eur. Phys. J. C \textbf{76}, no.8, 434 (2016)
%doi:10.1140/epjc/s10052-016-4271-x
[arXiv:1605.05081 [hep-ex]].

\bibitem{BaBar:2009hkt}
B.~Aubert \textit{et al.} [BaBar],
%``Searches for Lepton Flavor Violation in the Decays tau+- ---\ensuremath{>} e+- gamma and tau+- ---\ensuremath{>} mu+- gamma,''
Phys. Rev. Lett. \textbf{104}, 021802 (2010)
%doi:10.1103/PhysRevLett.104.021802
[arXiv:0908.2381 [hep-ex]].

\bibitem{Crivellin:2018qmi}
A.~Crivellin, M.~Hoferichter and P.~Schmidt-Wellenburg,
%``Combined explanations of $(g-2)_{\mu,e}$ and implications for a large muon EDM,''
Phys. Rev. D \textbf{98} (2018) no.11, 113002
%doi:10.1103/PhysRevD.98.113002
[arXiv:1807.11484 [hep-ph]].

\bibitem{Lindner:2016bgg}
M.~Lindner, M.~Platscher and F.~S.~Queiroz,
%``A Call for New Physics : The Muon Anomalous Magnetic Moment and Lepton Flavor Violation,''
Phys. Rept. \textbf{731} (2018), 1-82
%doi:10.1016/j.physrep.2017.12.001
[arXiv:1610.06587 [hep-ph]].

\bibitem{Dorsner:2020aaz}
I.~Dor\v{s}ner, S.~Fajfer and S.~Saad,
%``$\mu \to e \gamma$  selecting scalar leptoquark solutions for the $(g-2)_{e,\mu}$ puzzles,''
Phys. Rev. D \textbf{102} (2020) no.7, 075007
%doi:10.1103/PhysRevD.102.075007
[arXiv:2006.11624 [hep-ph]].
%
\bibitem{Hue:2021xap}
L.~T.~Hue, H.~T.~Hung, N.~T.~Tham, H.~N.~Long and T.~P.~Nguyen,
%``Large (g-2)\ensuremath{\mu} and signals of decays eb\textrightarrow{}ea\ensuremath{\gamma} in a 3-3-1 model with inverse seesaw neutrinos,''
Phys. Rev. D \textbf{104} (2021) no.3, 033007
%doi:10.1103/PhysRevD.104.033007
[arXiv:2104.01840 [hep-ph]].

\bibitem{Hue:2021xzl}
L.~T.~Hue, A.~E.~C\'arcamo Hern\'andez, H.~N.~Long and T.~T.~Hong,
%``Heavy singly charged Higgs bosons and inverse seesaw neutrinos as origins of large (g\ensuremath{-}2)e,\ensuremath{\mu} in two Higgs doublet models,''
Nucl. Phys. B \textbf{984} (2022), 115962
%doi:10.1016/j.nuclphysb.2022.115962
[arXiv:2110.01356 [hep-ph]].

\bibitem{Hong:2022xjg}
T.~T.~Hong, N.~H.~T.~Nha, T.~P.~Nguyen, L.~T.~T.~Phuong and L.~T.~Hue,
%``Decays h \textrightarrow{} eaeb, eb \textrightarrow{} ea\ensuremath{\gamma}, and (g \ensuremath{-} 2)e,\ensuremath{\mu} in a 3-3-1 model with inverse seesaw neutrinos,''
PTEP \textbf{2022} (2022) no.9, 093B05
%doi:10.1093/ptep/ptac109
[arXiv:2206.08028 [hep-ph]].

\bibitem{Li:2022zap}
S.~Li, Z.~Li, F.~Wang and J.~M.~Yang,
%``Explanation of electron and muon g \ensuremath{-} 2 anomalies in AMSB,''
Nucl. Phys. B \textbf{983} (2022), 115927
%doi:10.1016/j.nuclphysb.2022.115927
[arXiv:2205.15153 [hep-ph]].

%%%%Updated refs.
\bibitem{Yu:2021suw}
B.~Yu and S.~Zhou,
%``General remarks on the one-loop contributions to the muon anomalous magnetic moment,''
Nucl. Phys. B \textbf{975}, 115674 (2022)
%doi:10.1016/j.nuclphysb.2022.115674
[arXiv:2106.11291 [hep-ph]].

\bibitem{Leveille:1977rc}
J.~P.~Leveille,
%``The Second Order Weak Correction to (G-2) of the Muon in Arbitrary Gauge Models,''
Nucl. Phys. B \textbf{137} (1978), 63-76
%doi:10.1016/0550-3213(78)90051-2



\bibitem{Lavoura:2003xp}
L.~Lavoura,
%``General formulae for f(1) ---\ensuremath{>} f(2) gamma,''
Eur. Phys. J. C \textbf{29} (2003), 191-195
%doi:10.1140/epjc/s2003-01212-7
[arXiv:hep-ph/0302221 [hep-ph]].

\bibitem{Passarino:1978jh}
G.~Passarino and M.~J.~G.~Veltman,
%``One Loop Corrections for e+ e- Annihilation Into mu+ mu- in the Weinberg Model,''
Nucl. Phys. B \textbf{160} (1979), 151-207
%doi:10.1016/0550-3213(79)90234-7

\bibitem{tHooft:1978jhc}
G.~'t Hooft and M.~J.~G.~Veltman,
%``Scalar One Loop Integrals,''
Nucl. Phys. B \textbf{153} (1979), 365-401
%doi:10.1016/0550-3213(79)90605-9

\bibitem{Hue:2017lak}
L.~T.~Hue, L.~D.~Ninh, T.~T.~Thuc and N.~T.~T.~Dat,
%``Exact one-loop results for $l_i \to l_j\gamma$ in 3-3-1 models,''
Eur. Phys. J. C \textbf{78} (2018) no.2, 128
%doi:10.1140/epjc/s10052-018-5589-3
[arXiv:1708.09723 [hep-ph]].



\bibitem{Hahn:1998yk}
T.~Hahn and M.~Perez-Victoria,
%``Automatized one loop calculations in four-dimensions and D-dimensions,''
Comput. Phys. Commun. \textbf{118} (1999), 153-165
%doi:10.1016/S0010-4655(98)00173-8
[arXiv:hep-ph/9807565 [hep-ph]].

\bibitem{Denner:2016kdg}
A.~Denner, S.~Dittmaier and L.~Hofer,
%``Collier: a fortran-based Complex One-Loop LIbrary in Extended Regularizations,''
Comput. Phys. Commun. \textbf{212} (2017), 220-238
%doi:10.1016/j.cpc.2016.10.013
[arXiv:1604.06792 [hep-ph]].

\bibitem{Jurciukonis:2021izn}
D.~Jur\v{c}iukonis and L.~Lavoura,
%``Two-body lepton-flavour-violating decays in a 2HDM with soft family-lepton-number breaking,''
JHEP \textbf{03} (2022), 106
%doi:10.1007/JHEP03(2022)106
[arXiv:2107.14207 [hep-ph]].



\bibitem{Gunion:1989we}
J.~F.~Gunion, H.~E.~Haber, G.~L.~Kane and S.~Dawson,
``The Higgs Hunter's Guide,''
Front. Phys. \textbf{80} (2000), 1-404
SCIPP-89/13.


\bibitem{Bunk:2013uea}
D.~Bunk, J.~Hubisz and B.~Jain,
%``Higgs Decays in Gauge Extensions of the Standard Model,''
Phys. Rev. D \textbf{89} (2014) no.3, 035014
%doi:10.1103/PhysRevD.89.035014
[arXiv:1309.7988 [hep-ph]].

\bibitem{Hue:2017cph}
L.~T.~Hue, A.~B.~Arbuzov, T.~T.~Hong, T.~P.~Nguyen, D.~T.~Si and H.~N.~Long,
%``General one-loop formulas for decay $h\rightarrow Z\gamma $,''
Eur. Phys. J. C \textbf{78} (2018) no.11, 885
%doi:10.1140/epjc/s10052-018-6349-0
[arXiv:1712.05234 [hep-ph]].

\bibitem{Phan:2021xwc}
K.~H.~Phan, L.~Hue and D.~T.~Tran,
%``General one-loop contributions to the decay $H\rightarrow \nu_l\bar{\nu}_l\gamma$,''
PTEP \textbf{2021} (2021) no.10, 103B07
%doi:10.1093/ptep/ptab121
[arXiv:2106.14466 [hep-ph]].

\bibitem{VanOn:2021myp}
V.~Van On, D.~T.~Tran, C.~L.~Nguyen and K.~H.~Phan,
%``General one-loop formulas for $H\rightarrow f\bar{f}\gamma $ and its applications,''
Eur. Phys. J. C \textbf{82} (2022) no.3, 277
%doi:10.1140/epjc/s10052-022-10225-z
[arXiv:2111.07708 [hep-ph]].

\bibitem{Vermaseren:2000nd}
J.~A.~M.~Vermaseren,
``New features of FORM,''
[arXiv:math-ph/0010025 [math-ph]].


 \bibitem{Biggio:2016wyy}
C.~Biggio, M.~Bordone, L.~Di Luzio and G.~Ridolfi,
%``Massive vectors and loop observables: the $g-2$ case,''
JHEP \textbf{10} (2016), 002
%doi:10.1007/JHEP10(2016)002
[arXiv:1607.07621 [hep-ph]].

\bibitem{Barbieri:2015yvd}
R.~Barbieri, G.~Isidori, A.~Pattori and F.~Senia,
%``Anomalies in $B$-decays and $U(2)$ flavour symmetry,''
Eur. Phys. J. C \textbf{76} (2016) no.2, 67
%doi:10.1140/epjc/s10052-016-3905-3
[arXiv:1512.01560 [hep-ph]].


\bibitem{Peskin:1995ev}
M.~E.~Peskin and D.~V.~Schroeder,
 ``An Introduction to quantum field theory,''
Addison-Wesley, 1995,
ISBN 978-0-201-50397-5

\bibitem{Escribano:1996wp}
R.~Escribano and E.~Masso,
%``Improved bounds on the electromagnetic dipole moments of the $\tau$ lepton,''
Phys. Lett. B \textbf{395} (1997), 369-372
%doi:10.1016/S0370-2693(97)00059-2
[arXiv:hep-ph/9609423 [hep-ph]].

\bibitem{Eidelman:2016aih}
S.~Eidelman, D.~Epifanov, M.~Fael, L.~Mercolli and M.~Passera,
%``$\tau$ dipole moments via radiative leptonic $\tau$ decays,''
JHEP \textbf{03} (2016), 140
%doi:10.1007/JHEP03(2016)140
[arXiv:1601.07987 [hep-ph]].
%Cheng:1985bj
\bibitem{Cheng:1984vwu}
T.~P.~Cheng and L.~F.~Li,
 ``Gauge theory of elementary particle physics,''
Oxford University Press, 1984,
ISBN 978-0-19-851961-4, 978-0-19-851961-4

\bibitem{Freitas:2014pua}
A.~Freitas, J.~Lykken, S.~Kell and S.~Westhoff,
%``Testing the Muon g-2 Anomaly at the LHC,''
JHEP \textbf{05} (2014), 145
[erratum: JHEP \textbf{09} (2014), 155]
%doi:10.1007/JHEP09(2014)155
[arXiv:1402.7065 [hep-ph]].

\bibitem{Stockinger:2006zn}
D.~Stockinger,
%``The Muon Magnetic Moment and Supersymmetry,''
J. Phys. G \textbf{34} (2007), R45-R92
%doi:10.1088/0954-3899/34/2/R01
[arXiv:hep-ph/0609168 [hep-ph]].

\bibitem{tHooft:1972tcz}
G.~'t Hooft and M.~J.~G.~Veltman,
%``Regularization and Renormalization of Gauge Fields,''
Nucl. Phys. B \textbf{44} (1972), 189-213
%doi:10.1016/0550-3213(72)90279-9

\bibitem{Hue:2015fbb}
L.~T.~Hue, H.~N.~Long, T.~T.~Thuc and T.~Phong Nguyen,
%``Lepton flavor violating decays of Standard-Model-like Higgs in 3-3-1 model with neutral lepton,''
Nucl. Phys. B \textbf{907} (2016), 37-76
%doi:10.1016/j.nuclphysb.2016.03.034
[arXiv:1512.03266 [hep-ph]].


\bibitem{Cornella:2019uxs}
C.~Cornella, P.~Paradisi and O.~Sumensari,
%``Hunting for ALPs with Lepton Flavor Violation,''
JHEP \textbf{01} (2020), 158
%doi:10.1007/JHEP01(2020)158
[arXiv:1911.06279 [hep-ph]].

\bibitem{Bauer:2019gfk}
M.~Bauer, M.~Neubert, S.~Renner, M.~Schnubel and A.~Thamm,
%``Axionlike Particles, Lepton-Flavor Violation, and a New Explanation of $a_\mu$ and $a_e$,''
Phys. Rev. Lett. \textbf{124} (2020) no.21, 211803
%doi:10.1103/PhysRevLett.124.211803
[arXiv:1908.00008 [hep-ph]].

\bibitem{Liu:2018xkx}
J.~Liu, C.~E.~M.~Wagner and X.~P.~Wang,
%``A light complex scalar for the electron and muon anomalous magnetic moments,''
JHEP \textbf{03} (2019), 008
%doi:10.1007/JHEP03(2019)008
[arXiv:1810.11028 [hep-ph]].






 %\bibitem{JCRomao} J. C. Romao, Advanced Quantum Field Theory (IST, 2019), Available online at
 %http://porthos.tecnico.ulisboa.pt/Public/textos/tca.pdf.
 
 
 \bibitem{Djouadi:1996yq}
 A.~Djouadi, V.~Driesen, W.~Hollik and A.~Kraft,
 %``The Higgs photon - Z boson coupling revisited,''
 Eur. Phys. J. C \textbf{1} (1998), 163-175
% doi:10.1007/BF01245806
 [arXiv:hep-ph/9701342 [hep-ph]].
 
 \bibitem{Ashanujjaman:2021txz}
 S.~Ashanujjaman and K.~Ghosh,
 %``Revisiting type-II see-saw: present limits and future prospects at LHC,''
 JHEP \textbf{03} (2022), 195
 %doi:10.1007/JHEP03(2022)195
 [arXiv:2108.10952 [hep-ph]].
 

